Towards Human-Centered Early Prediction Models for Academic Performance in Real-World Contexts

Supporting student success requires collaboration among multiple stakeholders. Researchers have explored machine learning models for academic performance prediction; yet key challenges remain in ensuring these models are interpretable, equitable, and actionable within real-world educational support systems. First, many models prioritize predictive accuracy but overlook human-centered machine learning principles, limiting trust among students and reducing their usefulness for educators and institutional decision-makers. Second, most models require at least a month of data before making reliable predictions, delaying opportunities for early intervention. Third, current models primarily rely on sporadically collected, classroom-derived data, missing broader behavioral patterns that could provide more continuous and actionable insights. To address these gaps, we present three modeling approaches-LR, 1D-CNN, and MTL-1D-CNN-to classify students as low or high academic performers. We evaluate them based on explainability, fairness, and generalizability to assess their alignment with key social values. Using behavioral and self-reported data collected within the first week of two Spring terms, we demonstrate that these models can identify at-risk students as early as week one. However, trade-offs across human-centered machine learning principles highlight the complexity of designing predictive models that effectively support multi-stakeholder decision-making and intervention strategies. We discuss these trade-offs and their implications for different stakeholders, outlining how predictive models can be integrated into student support systems. Finally, we examine broader socio-technical challenges in deploying these models and propose future directions for advancing human-centered, collaborative academic prediction systems.

==> fig_tab/MTL_architecture.tex <==
\begin{figure}[!htb]
    \centering
\includegraphics[scale=0.30]{figures/MTL_architecture.png}
    \caption{Architecture of Multi-task Learning. The figure shows the architectural overview of our multi-task learning model that is more generalizable and deployable and outperforms all other baselines. The green boxes represent the shared hidden layers in the model.} 
    \label{fig:architecture}
\end{figure}

==> fig_tab/MTL_methods.tex <==
\begin{figure}[htb!]
    \centering
     \subfloat[Hard parameter sharing]{\includegraphics[scale=0.27]{figures/hard parameter sharing.png}\label{fig:hard_param}}
     \subfloat[Soft parameter sharing]{\includegraphics[scale=0.27]{figures/soft parameter sharing.png}\label{fig:soft_param}}
     
    \caption{Two commonly used Multi-Task Learning methods.} 
    \label{fig:MTL_methods}
\end{figure}


==> fig_tab/MTLfairness_plot_2019.tex <==
\begin{figure}[htb!]
    \centering
     \subfloat[Race]{\includegraphics[scale=0.27]{figures/MTLfairness_race_2019.png}\label{fig:MTL_race_2019}}
     \subfloat[First-gen college student]{\includegraphics[scale=0.27]{figures/MTLfairness_1stGen_2019.png}\label{fig:MTL_1st_gen_2019}}
     
     \subfloat[Gender]{\includegraphics[scale=0.27]{figures/MTLfairness_gender_2019.png}\label{fig:MTL_gender_2019}}
     \subfloat[Sexual Orientation]{\includegraphics[scale=0.27]{figures/MTLfairness_sexual_2019.png}\label{fig:MTL_sexual_2019}}
    \caption{Visualization of grouped fairness metrics for four sensitive attributes on 2019 data.
    } 
    \label{fig:MTL_fairness_plot_2019}
\end{figure}


==> fig_tab/baseline_model_selection.tex <==
\begin{table}[htb!]
\scalebox{0.85}{
    \centering
     \begin{tabular}{c c c c c c c c}
        \toprule[1pt]
        \hline
        \textbf{Classifier} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{AUC} & \textbf{Kappa} & \makecell[c]{\textbf{Balanced}\\ \textbf{ accuracy}}\\\hline
        Logistic Regression & 0.229 & 0 & 0 & 0 & 0.571 & 0 & 0.500 \\
        KNN & 0.229 & 0 & 0 & 0 & 0.065 & 0 & 0.500 \\
        AdaBoost & 0.734 & 0.92 & 0.717 & 0.806 & 0.81 & 0.403 & 0.754\\
        Decision Tree & 0.739 & 0.869 & 0.779 & 0.822 & 0.713 & 0.342 & 0.692 \\
        Gradient Boosting & 0.745 & 0.882 & 0.772 & 0.824 & 0.811 & 0.369 & 0.712 \\
        Random Forest & 0.750 & 0.871 & 0.793 & 0.830 & 0.800 & 0.360 & 0.699 \\
        XGBoost & 0.771 & 0.911 & 0.779 & 0.840 & 0.810 & 0.447 & 0.762 \\\hdashline 
             \textbf{LSTM \cite{chen2020utilizing}} & \textbf{0.737} & \textbf{0.833} & \textbf{0.769} & \textbf{0.800} & \textbf{0.417} & \textbf{0.417} & \textbf{0.718} \\
        \textbf{SVM} & \textbf{0.766} & \textbf{0.955} & \textbf{0.731} & \textbf{0.828} & \textbf{0.834} & \textbf{0.481} & \textbf{0.807}\\\hline
         \bottomrule[1pt]
    \end{tabular}
    }
    \caption{Baseline Models. LSTM and SVM are selected, based on kappa and balanced accuracy.}
    \label{tab:model_selection}
\end{table}

% \renewcommand{\arraystretch}{1.2}
% \begin{table}[htb!]
%     \centering
%     \setlength{\tabcolsep}{1.2mm}{
%     \subfloat[Selecting predictive model using data from the first week of the 2018 Spring term.]{
%     \scalebox{0.85}{
%         \begin{tabular}{c c c c c c c c}
%         \toprule[1pt]
%         \hline
%         \textbf{Classifier} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{AUC} & \textbf{Kappa} & \makecell[c]{\textbf{Balanced}\\ \textbf{ accuracy}}\\\hline
%         KNN & 0.229 & 0.000 & 0.000 & 0.000 & 0.387 & 0.000 & 0.500 \\
%         SVM & 53.7\% & 0.73 & 0.634 & 0.679 & 0.444 & -0.135 & 42.2\% \\
%         Decision Tree & 58.5\% & 0.772 & 0.655 & 0.709 & 0.502 & 0.003 & 0.502 \\
%         AdaBoost & 0.617 & 0.759 & 0.738 & 0.748 & 0.424 & -0.051 & 0.474 \\
%         Gradient Boosting & 0.691 & 0.784 & 0.828 & 0.805 & 0.546 & 0.064 & 0.530 \\
%         XGBoost & 0.702 & 0.78 & 0.855 & 0.816 & 0.543 & 0.047 & 52.1\%  \\
%         Random Forest & 0.729 & 0.783 & 0.897 & 0.836 & 0.587 & 0.072 & 0.530 \\
%         \hdashline 
%         \textbf{Logistic Regression} & \textbf{0.915} & \textbf{0.901} & \textbf{1.000} & \textbf{0.948} & \textbf{0.962} & \textbf{0.722} & \textbf{0.814}\\\hline
%          \bottomrule[1pt]
%     \end{tabular}}\label{tab:model_per1}}%
%     \vspace{0.5cm}
    
%      \subfloat[Selecting 1R baseline model using a single feature, prior Winter term GPA.]{
%      \scalebox{0.80}{
%      \begin{tabular}{c c c c c c c c}
%         \toprule[1pt]
%         \hline
%         \textbf{Classifier} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{AUC} & \textbf{Kappa} & \makecell[c]{\textbf{Balanced}\\ \textbf{ accuracy}}\\\hline
%         Logistic Regression & 0.229 & 0.000 & 0.000 & 0.000 & 0.571 & 0 & 0.500 \\
%         KNN & 22.9\% & 0.000 & 0.000 & 0.000 & 0.065 & 0 & 0.500 \\
%         AdaBoost & 73.4\% & 0.92 & 0.717 & 0.806 & 0.81 & 0.403 & 0.754 \\
%         Decision Tree & 0.739 & 0.869 & 0.779 & 0.822 & 0.713 & 0.342 & 0.692 \\
%         Gradient Boosting & 0.745 & 0.882 & 0.772 & 0.824 & 0.811 & 0.369 & 0.712 \\
%         Random Forest & 0.750 & 0.871 & 0.793 & 0.830 & 0.800 & 0.360 & 0.699 \\
%         XGBoost & 0.771 & 0.911 & 0.779 & 0.840 & 0.810 & 0.447 & 0.762 \\\hdashline 
%         \textbf{LSTM} & \textbf{0.737} & \textbf{0.833} & \textbf{0.769} & \textbf{0.800} & \textbf{0.417} & \textbf{0.417} & \textbf{0.718} \\
%         \textbf{SVM} & \textbf{0.766} & \textbf{0.955} & \textbf{0.731} & \textbf{0.828} & \textbf{0.834} & \textbf{0.481} & \textbf{0.807}\\\hline
%          \bottomrule[1pt]
%     \end{tabular}}\label{tab:model_per2}}%
%     }
%     \caption{Performance of eight machine learning classifiers. Logistic Regression is selected, based on all performance metrics, as our predictive model. LSTM and SVM are selected, based on kappa and balanced accuracy, as 1R baseline model.}
%     \label{tab:model_performance}
% \end{table}
% \renewcommand{\arraystretch}{1.0}

==> fig_tab/breakpoint.tex <==
\begin{figure}[h]
\scalebox{0.70}{
    \centering
\includegraphics[scale=0.5]{figures/breakpoint_illustration.png}}
    \caption{Participant's behavior change in screen usage and breakpoint visualization.} 
    \label{fig:breakpoint}
\end{figure}


==> fig_tab/demographics.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}[htb!]
\scalebox{0.85}{
    \begin{tabular}{c|lccccccc}\toprule[1pt]\hline
    \multirow{2}{*}{\textbf{Year}} && \multirow{2}{*}{\textbf{Protected Attribute}}&&\multicolumn{2}{c}{\textbf{Protected Group}}&&\multicolumn{2}{c}{\textbf{Unprotected Group}} \\
    \cline{5-6}\cline{8-9}
    && && number (\% in A/\% in G)  & mean (std) && number (\% in A/\% in G)  & mean (std)  \\\hline
    \multirow{4}{*}{2018} && \makecell[l]{Race} &&  32 (17.0\%/37.5\%) &  3.27 (0.61)  && 156 (83.0\%/19.9\%)  &  3.52 (0.42)   \\\cline{2-9}
    && \makecell[l]{First-generation} && 57 (30.3\%/33.3\%)  &  3.34 (0.50)  &&  131 (69.7\%/18.3\%) &  3.54 (0.44)    \\\cline{2-9}
    && \makecell[l]{Gender} &&  123 (65.4\%/24.4\%) &  3.63 (0.39)  &&  65 (34.5\%/20.0\%) &   3.46 (0.48) \\\cline{2-9}
    && \makecell[l]{Sexual Orientation} &&  21 (11.2\%/14.3\%) &  3.46 (0.49)  &&  167 (88.8\%/24.0\%) &  3.52 (0.42)    \\\hline
    \multirow{4}{*}{2019} && \makecell[l]{Race} &&  23 (11.7\%/52.2\%) &  3.00 (0.77)  &&  173 (88.3\%/29.5\%) &   3.36 (0.56) \\\cline{2-9}
    && \makecell[l]{First-generation} &&  58 (29.6\%/44.8\%) &   3.12 (0.64) &&  138 (70.4\%/26.8\%) &  3.40 (0.57)  \\\cline{2-9}
    && \makecell[l]{Gender} && 100 (51.0\%/35\%)  &  3.38 (0.60)  && 96 (49.0\%/29.2\%)  &   3.31 (0.61) \\\cline{2-9}
    && \makecell[l]{Sexual Orientation} &&  21 (10.7\%/23.8\%) &  3.25 (0.69)  &&  175 (89.3\%/33.1\%) &   3.39 (0.49)  \\\hline
    \bottomrule                 
\end{tabular}}
\caption{Demographics (total number, percentage in each protect attribute, and percentage of low performers in that group) and statistics (mean and standard deviations) of 2018 and 2019 Spring term GPAs for four protected attributes (race, first-generation college student, gender, and sexual orientation). Underrepresented minority, first-generation college students, gender other than male (including female and transgender), and sexual minority (such as homosexual and bisexual) are protected groups for gender, first-generation, race, and sexual orientation. \% in A represents for the percentage of that group in each attribute, while \% in G represents for the percentage of low performers in that group.}
\label{tab:demographics}
\end{table}
\renewcommand{\arraystretch}{1.2}


==> fig_tab/fairness_demographics.tex <==
\renewcommand{\arraystretch}{1.2}
    \begin{table}[htb!]
    \scalebox{0.85}{
\begin{tabular}{lccccccc}\toprule[1pt]\hline
             \multirow{2}{*}{\textbf{Protected Attribute}}&&\multicolumn{2}{c}{\textbf{2018 (n=188)}}&&\multicolumn{2}{c}{\textbf{2019 (n=196)}} \\ %&&\multirow{2}{*}{\makecell[c]{\textbf{US Census} \\ (MG \%)}} \\
             \cline{3-4}\cline{6-7}
             && MG  & Non-MG && MG & Non-MG \\
             \hline
    Race  && 32 (17.0\%) & 156 (83.0\%) && 23 (11.7\%) & 173 (88.3\%)\\\hline %&& $\approx$ 17.9\% \cite{census_race}\\\hline
    First-generation  &&  57 (30.3\%) &  131 (69.7\%) &&  58 (29.6\%) &  138 (70.4\%) \\\hline %&& $\approx$ 33.3\% \cite{first-generation}\\\hline
    Gender  && 123 (65.4\%)  &  65 (34.5\%) && 100 (51.0\%) & 96 (49.0\%) \\\hline %&& $\approx$ 54.3\% \cite{census_gender}\\\hline
    Sexual Orientation  &&  21 (11.2\%) &  167 (88.2\%) &&  21 (10.7\%) & 175 (89.3\%)\\\hline %&& $\approx$ 7.1\% \cite{census_lgbtq}\\\hline
    \bottomrule                               
\end{tabular}}
\caption{Statistics of four protected attributes (race, first-generation college student, gender, and sexual orientation). MG represents for minority group, while Non-MG referents for non-minority group.} %\han{The credibility of these census data sources needs to be carefully checked.}}%Gender minority includes all genders other than man (including female and transgender). Race minority is underrepresented minority. Sexual minority includes all non-heterosexual participants.}
\label{tab:fairness_demographics}
\end{table}
\renewcommand{\arraystretch}{1.2}

==> fig_tab/fairness_plot_2018.tex <==
\begin{figure}[htb!]
    \centering
     \subfloat[Race]{\includegraphics[scale=0.27]{figures/fairness_race_2018.png}\label{fig:race_2018}}
     \subfloat[First-gen college student]{\includegraphics[scale=0.27]{figures/fairness_1stGen_2018.png}\label{fig:1st_gen_2018}}
     
     \subfloat[Gender]{\includegraphics[scale=0.27]{figures/fairness_gender_2018.png}\label{fig:gender_2018}}
     \subfloat[Sexual Orientation]{\includegraphics[scale=0.27]{figures/fairness_sexual_2018.png}\label{fig:sexual_2018}}
    \caption{Visualization of grouped fairness metrics on four sensitive attributes in 2018.
    } 
    \label{fig:fairness_plot_2018}
\end{figure}


==> fig_tab/gpa_comparison.tex <==
\renewcommand{\arraystretch}{1.0}
\begin{table}[htb!]
    \small
    \centering
    \scalebox{0.9}{\setlength{\tabcolsep}{1.2mm}{
    \begin{tabular}{lccccc}
    \toprule[1pt]
    \hline
    \textbf{Test} & \textbf{Year} & \makecell[c]{\textbf{Minority group} \\\textbf{Mean $\pm$ SD}} & \makecell[c]{\textbf{Non-minority group} \\ \textbf{Mean $\pm$ SD}} & \textbf{t} & \textbf{p value} \\ \hline
    \multirow{2}{*}{Test 1 (Race)} & 2018 & 3.27 $\pm$ 0.61 & 3.52 $\pm$ 0.42 & -2.26 & .029* \\ \cline{2-6} 
    & 2019 & 3.00 $\pm$ 0.77 & 3.36 $\pm$ 0.56 & -2.31 & 0.028* \\ \hline
    \multirow{2}{*}{Test 2 (First-generation)} & 2018 & 3.34 $\pm$ 0.50 & 3.54 $\pm$ 0.44 & -2.65 & 0.009** \\ \cline{2-6} 
    & 2019 & 3.12 $\pm$ 0.64 & 3.40 $\pm$ 0.57 & -2.97 & 0.004** \\ \hline
    \multirow{2}{*}{Test 3 (Gender)} & 2018 & 3.63 $\pm$ 0.39 & 3.46 $\pm$ 0.48 & 1.89 & 0.068 \\ \cline{2-6} 
    & 2019 & 3.38 $\pm$ 0.60 & 3.31 $\pm$ 0.61 & 0.51 & 0.611 \\ \hline
    \multirow{2}{*}{Test 4 (Sexual Orientation)} & 2018 & 3.46 $\pm$ 0.49 & 3.52 $\pm$ 0.42 & -0.84 & 0.403 \\ \cline{2-6} 
    & 2019 & 3.25 $\pm$ 0.69 & 3.39 $\pm$ 0.49 & -1.68 & 0.095 \\ \hline
    \bottomrule[1pt]
    \end{tabular}}}
    \caption{Means and standard deviations of 2018 and 2019 Spring term GPAs of interest for different minoritized student groups. Test 1 is conducted between Underrepresented minority and non-underrepresented minority. Test 2 is conducted between first-generation students and non first-generation students. Test 3 is conducted between gender other than male (including female and transgender) and male. Test 4 is conducted between sexual minority (such as homosexual and bisexual) and non-sexual minority. T-test values and significance levels are indicated. Significance is marked as * $p$<.05, ** $p$<.01, *** $p$<.001. }
    \label{tab:gpa_comparison}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> fig_tab/related_work_old.tex <==
\begin{centering}
    \scriptsize
    \setlength{\tabcolsep}{1.5mm}{
\begin{table}[h]
\scalebox{0.75}{
    % \begin{tabular}{p{5mm} p{9mm} p{2.5cm} p{5cm}  p{3cm} p{3cm}}
    \begin{tabular}{m{0.02\textwidth} c m{0.09\textwidth} m{0.30\textwidth} m{0.20\textwidth} m{0.25\textwidth} c c}
    \hline\hline
 \multicolumn{8}{c}{\textbf{\large Detection}} \\ % align: l,c,r
\hline
    & \multicolumn{1}{c}{\textbf{Data}} & \multicolumn{1}{c}{\textbf{Task}} & \multicolumn{1}{c}{\textbf{Input}}  &
    \multicolumn{1}{c}{\textbf{Models}} & \multicolumn{1}{c}{\textbf{Metrics}} &
    \multicolumn{1}{c}{\textbf{G Eval}} &
    \multicolumn{1}{c}{\makecell[c]{\textbf{Model}\\\textbf{Int.}}}
    \\\hline
        \cite{Nghe07}  & Year & End-of-year GPA (2-class, 3-class \& 4-class)  & 
        Student records and demographics (\eg gender; institute rank;  income), academics (\eg cumulative GPA)
         & Decision tree; Bayesian network & Accuracy = 71-73\% (4-class); 74-86\% (3-class); 93-94\% (2-class)& $\times$ & $\times$ \\\hline
    
\cite{yao2019predicting} & Term  & Term GPA (continuous) & Campus smart card logs (\eg location use), academics (\eg grades; credits) & MTL-based Algorithm  &  Average $r$=0.433, SD=0.007   \\\hline
\cite{wang2015smartgpa}   & 10 wks & Cumulative GPA (continuous)  &  Behavioral data (\eg sleep; location; mobility); self-reports (\eg affect; stress; mood); academics   (\eg class attendance) & Linear regression with lasso regularization & MAE = 0.179,  $r$ = 0.81, $R^2$ = 0.559 \\
\hline\hline
\multicolumn{8}{c}{
\textbf{\Large Prediction}}\\ % align: l,c,r
\hline & 
    \multicolumn{1}{c}{\textbf{Time}} & \multicolumn{1}{c}{\textbf{Task}} & \multicolumn{1}{c}{\textbf{Input}}  &
    \multicolumn{1}{c}{\textbf{Models}} & \multicolumn{1}{c}{\textbf{Metrics}} &
    \multicolumn{1}{c}{\textbf{G Eval}}&
    \multicolumn{1}{c}{\makecell[c]{\textbf{Model}\\\textbf{Int.}}}  \\\hline

   \cite{sukhbaatar2019artificial}  & 13 wks  & Term GPA (2-class) & Learning Management System Log data (\eg online activity data); academics (\eg class final grades) & Neural Network &  Avg accuracy $\approx$ 92\%, avg sensitivity = 65\%, avg precision $\approx$ 75\%, avg F1 = 66\% \\\hline
   \cite{lara2014system} &   10 wks  & Term GPA \mbox{(2-class)} & Online Learning Log data (\eg logins, resources viewed) & Clustering Algorithm & Accuracy = 94\%,  precision = 0.818,  recall = 0.9, specificity = 0.95  \\\hline
   \cite{lu2018applying} & 6 wks &  Term GPA (continuous) & Hybrid Learning Log Data (\eg video watching; online practice); academics (\eg weekly scores; tutoring participation) & Principle component regression & Predictive MSE=159.71,  predictive mean absolute percentage correction = 82\%; $R^2$=0.56\\\hline
   \cite{yu2018improving} & 5  wks & Term GPA (simplified 2-class) & Academics (\eg attendance; in-class participation; homework completion;  grades); self reflections (\eg detected sentiment) & CNN  & Accuracy = 71\%, F1 = 0.71 \\ \hline 
   \cite{sano2015recognizing} & Month & Term GPA (2-class) & Behavioral data (\eg calls; location; sleep); self-reports (\eg PSQI; PSS); academic performance  & SVM-L/SVL-RBF & Accuracy: 88\% to 92\% for top performing features ACC and PHONE, respectively\\\hline
   \cite{chen2020utilizing} & Month & Term GPA (2-class) & Learning Management System Log data (\eg online activity timing and location by activity type) & LSTM & AUC = 0.616 and 0.596 on two test sets \\\hdashline
   Our work & 1 wk  & Term GPA  (2-class) & Behavioral data (\eg phone use; sleep; steps); self-reports (\eg social media use; unfair treatment; mental health);  academics (\eg  class attendance; number of courses taken; prior GPA)); student records and demographics (\eg gender; race; sexuality) & Logistic Regression with L2 (Ridge) regularization & Accuracy = 89.3\%, precision = 0.894, recall = 0.955, F1 = 0.924, AUC = 0.796, Kappa = 0.745, Balanced acc = 85.8\% \\\hline
   \bottomrule[1pt]
   \end{tabular}}
   \caption{Related work  sorted by amount of  (\textbf{Data}) \textit{needed for detection/prediction.} The prediction \textbf{Task} is either classifying students into groups  (such as below and above 3.2, in our case) or regression (continues GPA) All papers focus on end-of-term GPA except \cite{Nghe07}, which detects end-of-year GPA and \cite{wang2015smartgpa}, which detects cumulative GPA.  The data set used as \textbf{Input} for each paper varied greatly and included, variously, demographics, student records, behavioral data, self reports, and logs of online learning system use; the type of machine learning \textbf{Model} and the \textbf{Metrics} for assessing the model also varied significantly, making comparison difficult.} 
   \label{tab:related_work}
\end{table}}
\end{centering}

==> fig_tab/service_provider.tex <==
\begin{figure}[h]
    \centering
    \scalebox{1}{
    \includegraphics[width=0.5\textwidth]{figures/service_provider.pdf}}
    \caption{Distribution of service providers in 2018.}
    \label{fig:service_provider}
\end{figure}

==> fig_tab/variables.tex <==
\newcommand{\pItotalGPAnumber}{195}
\newcommand{\pItotalparticipants}{209}
\newcommand{\pIItotalparticipants}{253}
\newcommand{\pIIItotalparticipants}{162}
\newcommand{\pIdroppedout}{x}
\newcommand{\pIIdroppedout}{x}
\newcommand{\pIIIdroppedout}{x}
\newcommand{\pItotalremains}{195}
\newcommand{\pIItotalremains}{201}
\newcommand{\pIIItotalremains}{119}
\newcommand{\pIvalidparticipants}{188}
\newcommand{\pIIvalidparticipants}{196}
\newcommand{\pIIIvalidparticipants}{x}

\newcommand{\pIstarttime}{March 26}
\newcommand{\pIIstarttime}{April 1}
\newcommand{\pIIIstarttime}{March 30}
\newcommand{\pIendtime}{June 03}
\newcommand{\pIIendtime}{June 07}
\newcommand{\pIIIendtime}{June 05}
\newcommand{\compensation}{245}

